Explicit solution to dynamic portfolio choice problem : The continuous-time detour

This paper solves the dynamic portfolio choice problem. Using an explicit solution with a power utility, we construct a bridge between a continuous and discrete VAR model to assess portfolio sensitivities. We find, from a well analyzed example that the optimal allocation to stocks is particularly sensitive to Sharpe ratio. Our quantitative analysis highlights that this sensitivity increases when the risk aversion decreases and/or when the time horizon increases. This finding explains the low accuracy of discrete numerical methods especially along the tails of the unconditional distribution of the state variable.

==> explicit-solution-tab1.tex <==
10 & LT & \num{0.0} & \num{6.5} & \num{42.1} & \num{77.7} & \num{100.0} & \num{0.0} & \num{2.5} & \num{15.2} & \num{27.9} & \num{46.3} \tabularnewline
 & GS & \num{0.0} & \num{13.3} & \num{43.2} & \num{73.1} & \num{100.0} & \num{0.0} & \num{4.3} & \num{15.4} & \num{27.0} & \num{44.7} \tabularnewline
 & $𝛥$ & \num{0.0} & \num{-6.8} & \num{-1.1} & \num{4.6} & \num{0.0} & \num{0.0} & \num{-1.8} & \num{-0.2} & \num{0.9} & \num{1.6} \tabularnewline
\midrule
20 & LT & \num{0.0} & \num{13.7} & \num{57.8} & \num{100.0} & \num{100.0} & \num{0.0} & \num{5.9} & \num{22.8} & \num{39.7} & \num{64.1} \tabularnewline
 & GS & \num{0.0} & \num{24.4} & \num{57.2} & \num{89.7} & \num{100.0} & \num{0.0} & \num{10.7} & \num{25.1} & \num{40.4} & \num{63.2} \tabularnewline
 & $𝛥$ & \num{0.0} & \num{-10.7} & \num{0.6} & \num{10.3} & \num{0.0} & \num{0.0} & \num{-4.8} & \num{-2.3} & \num{-0.7} & \num{0.9} \tabularnewline
\midrule
30 & LT & \num{0.0} & \num{22.8} & \num{73.2} & \num{100.0} & \num{100.0} & \num{0.0} & \num{10.8} & \num{31.5} & \num{52.1} & \num{81.9} \tabularnewline
 & GS & \num{0.0} & \num{32.8} & \num{68.4} & \num{100.0} & \num{100.0} & \num{0.0} & \num{17.5} & \num{35.2} & \num{54.0} & \num{80.7} \tabularnewline
 & $𝛥$ & \num{0.0} & \num{-10.0} & \num{4.8} & \num{0.0} & \num{0.0} & \num{0.0} & \num{-6.7} & \num{-3.7} & \num{-1.9} & \num{1.2} \tabularnewline
\midrule
40 & LT & \num{0.0} & \num{32.0} & \num{86.9} & \num{100.0} & \num{100.0} & \num{0.0} & \num{16.5} & \num{40.2} & \num{64.0} & \num{98.3} \tabularnewline
 & GS & \num{0.0} & \num{38.8} & \num{77.6} & \num{100.0} & \num{100.0} & \num{0.0} & \num{24.1} & \num{44.5} & \num{65.7} & \num{94.6} \tabularnewline
 & $𝛥$ & \num{0.0} & \num{-6.8} & \num{9.3} & \num{0.0} & \num{0.0} & \num{0.0} & \num{-7.6} & \num{-4.3} & \num{-1.7} & \num{3.7} \tabularnewline


==> explicit-solution-tab2.tex <==
10 & MD & \num{-34.0} & \num{3.0} & \num{28.6} & \num{54.2} & \num{91.1} & \num{-11.3} & \num{1.0} & \num{9.5} & \num{18.1} & \num{30.4} \tabularnewline
 & HD & \num{-10.9} & \num{3.5} & \num{13.5} & \num{23.6} & \num{38.0} & \num{-4.6} & \num{1.5} & \num{5.7} & \num{9.9} & \num{15.9} \tabularnewline
\midrule
20 & MD & \num{-34.0} & \num{3.0} & \num{28.6} & \num{54.2} & \num{91.1} & \num{-11.3} & \num{1.0} & \num{9.5} & \num{18.1} & \num{30.4} \tabularnewline
 & HD & \num{-15.9} & \num{10.8} & \num{29.2} & \num{47.7} & \num{74.3} & \num{-7.2} & \num{4.9} & \num{13.3} & \num{21.6} & \num{33.7} \tabularnewline
\midrule
30 & MD & \num{-34.0} & \num{3.0} & \num{28.6} & \num{54.2} & \num{91.1} & \num{-11.3} & \num{1.0} & \num{9.5} & \num{18.1} & \num{30.4} \tabularnewline
 & HD & \num{-16.0} & \num{19.8} & \num{44.7} & \num{69.5} & \num{105.3} & \num{-7.7} & \num{9.8} & \num{21.9} & \num{34.1} & \num{51.6} \tabularnewline
\midrule
40 & MD & \num{-34.0} & \num{3.0} & \num{28.6} & \num{54.2} & \num{91.1} & \num{-11.3} & \num{1.0} & \num{9.5} & \num{18.1} & \num{30.4} \tabularnewline
 & HD & \num{-13.2} & \num{29.1} & \num{58.3} & \num{87.6} & \num{129.8} & \num{-6.5} & \num{15.5} & \num{30.7} & \num{46.0} & \num{68.0} \tabularnewline

